Counterexample-Preserving Reduction for Symbolic Model Checking

The cost of LTL model checking is highly sensitive to the length of the formula under verification. We observe that, under some specific conditions, the input LTL formula can be reduced to an easier-to-handle one before model checking. In our reduction, these two formulae need not to be logically equivalent, but they share the same counterexample set w.r.t the model. In the case that the model is symbolically represented, the condition enabling such reduction can be detected with a lightweight effort (e.g., with SAT-solving). In this paper, we tentatively name such technique "Counterexample-Preserving Reduction" (CePRe for short), and finally the proposed technquie is experimentally evaluated by adapting NuSMV.

==> conc.tex <==

%-----------------------------------

\section{Concluding Remarks}
\label{Sec: Conclusion}

%-----------------------------------

In this paper, we present a new technique
to reduce  LTL specifications'
complexity towards  symbolic model checking,
namely, \cepre$\!\!$.
The novelty in this technique is that 
the formula being reduced need not to be
logically equivalent with the one after reduction,
but just need to preserve the counterexample set.
Moreover, the condition enabling such a reduction
can be usually detected with  lightweight approaches,
such as SAT-solving.
Hence, this technique could leverage the power of SAT-solvers.


The central part of  \cepre is a set of reduction rules,
and soundness of these reduction rules are fairly easy to check.
For the model dependent rules,
additional conditions mainly concern invariants and
transitions only, and we do not make
a sufficient use of other features, such as fairness.
In this paper, we just consider combinations of
two temporal operators as many as possible,
indeed, there might be other possible
reduction schemas we are not  aware.
Indeed, in this paper, we tentatively to provide such
a framework, and one can extend it to 
model checking of other logics.


From the experimental results, we can see that,
in a statistical perspective, we can gain a better 
performance and lower overhead
with \cepre$\!\!$.

